AdaptiveCoPilot: Design and Testing of a NeuroAdaptive LLM Cockpit Guidance System in both Novice and Expert Pilots

Pilots operating modern cockpits often face high cognitive demands due to complex interfaces and multitasking requirements, which can lead to overload and decreased performance. This study introduces AdaptiveCoPilot, a neuroadaptive guidance system that adapts visual, auditory, and textual cues in real time based on the pilot's cognitive workload, measured via functional Near-Infrared Spectroscopy (fNIRS). A formative study with expert pilots (N=3) identified adaptive rules for modality switching and information load adjustments during preflight tasks. These insights informed the design of AdaptiveCoPilot, which integrates cognitive state assessments, behavioral data, and adaptive strategies within a context-aware Large Language Model (LLM). The system was evaluated in a virtual reality (VR) simulated cockpit with licensed pilots (N=8), comparing its performance against baseline and random feedback conditions. The results indicate that the pilots using AdaptiveCoPilot exhibited higher rates of optimal cognitive load states on the facets of working memory and perception, along with reduced task completion times. Based on the formative study, experimental findings, qualitative interviews, we propose a set of strategies for future development of neuroadaptive pilot guidance systems and highlight the potential of neuroadaptive systems to enhance pilot performance and safety in aviation environments.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016
modified by Matt Brehmer, Feb 2024

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE VIS: Visualization & Visual Analytics (Short Papers, Posters)
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> hackstyle.tex <==
%\setlength{\titlespace}{0ex}
%\setlength{\titlespace}{1.0ex}
%\setlength{\textheight}{9.25in}
\setlength{\abovecaptionskip}{1.0ex}
\setlength{\belowcaptionskip}{1.0ex}
\setlength{\floatsep}{1.0ex}
\setlength{\dblfloatsep}{\floatsep}
\setlength{\textfloatsep}{2.0ex}
\setlength{\dbltextfloatsep}{\textfloatsep}
%\setlength{\intextsep}{1.0ex}
\setlength{\abovedisplayskip}{1.0ex}
\setlength{\belowdisplayskip}{1.0ex}
%\setlength{\arraycolsep}{1ex}
%\setlength{\parskip}{1.0ex} % actually increase space for acmart
%\setlength{\baselineskip}{1ex}
%\setlength{\teaserspace}{1ex}
%\linespread{1.0} % default 1.0; WMD! very evil, be very careful


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/9994_SystemDesign_Backup.tex <==
\section{\systemname Adaptivity}
\systemname is designed to provide adaptive guidance through text, audio, and interactive cues based on real-time assessments of the pilot’s cognitive load and performance. During pre-flight checks, pilots receive auditory, visual, and textual tips tailored to their cognitive state. The system dynamically adjusts the combination and quantity of these modalities depending on whether the cognitive load is sub-optimal (either too high or too low). This section outlines the design decisions behind our system, explains why these choices were made, identifies the challenges they pose, and describes how we address these challenges.

% \systemname aims to optimally present adaptive guidance in the form of text, audio, and interaction cues based on real-time pilot cognitive load levels and performance. As pilots conduct pre-flight checks, they receive auditory, visual, and textual tips. A sub-optimal (higher or lower) cognitive load leads to changes in the configuration of \textbf{how} modalities combine and changes in the amount of information they receive. The following sections will discuss the design decisions in our system, why we chose these designs, what challenges they introduce, and how we overcome them.

\begin{comment}
    \subsubsection{Adaptive Rules}
    - why adapt? why this works better than any other methods? 
    - why this is the right way to do?

    - how did we plan to do this? 
    - 7 rules
    
why do you use it? how do you use it? 
\end{comment}

\subsection{Guidance Adaptation Using Cognitive Workload Theories}
Our approach to adaptive guidance is neuroadaptive, meaning it adjusts based on cognitive workload theories to avoid overloading the pilot's attention, perception, or memory. We use 28 adaptive strategies, detailed in Appendix, and base our rules on the following three key cognitive workload theories and results from the formative study.
%We use a neuroadaptive approach to guidance adaption to provide guidance cues that provide meaningful information to the pilot without overloading attentionally, perceptually, or memory-wise. 
%To provide meaningful adaptive guidance we follow a set of cognitive workload theories from previous works.
%\textcolor{red}{Add in lit review}

%We use a total of 28 adaptive strategies detailed in appendix \cite{wickens2002multiple}. To summarize our general flow of adaptive we structure rules around these 3 cognitive workload theories.

\begin{itemize}
    \item Underload Scenarios: Provide more information and use diverse modalities (visual, audio, text) to stimulate engagement and prevent errors due to a lack of focus. \cite{sweller1988cognitive}
    \item Overload Scenarios: Reduce the information load and rely primarily on visual cues to help reduce cognitive overload and keep pilots calm and focused. \cite{spence1997audiovisual}
    \item Optimal Scenarios: Use a balanced mix of visual and audio prompts, providing enough information to assist the pilot while avoiding unnecessary distractions. \cite{parasuraman2008mitigating}
\end{itemize}

To ensure effective adaptive guidance, we align our system with these cognitive workload theories. For instance:

\myparagraph{Underload Scenarios} The system increases engagement by providing more detailed information and introducing diverse modalities. Visual, audio, and text prompts are used to stimulate the pilot’s focus and ensure they remain attentive during less demanding phases of flight. As cognitive demand is low, introducing additional complexity helps prevent errors due to a lack of attention. 
%The system uses frequent prompts and reminders to maintain engagement and prevent lapses in concentration, thus ensuring that the pilot remains fully aware of the aircraft's status and environmental factors.

\myparagraph{Optimal Scenarios} When the pilot’s cognitive load is in an optimal range, the system focuses on maintaining balance by providing a mixture of visual and audio prompts that are tailored to the task at hand. In these scenarios, the system aims to deliver just-in-time feedback, giving enough information to assist the pilot without causing distraction. 
%This balance allows the pilot to maintain situational awareness while efficiently completing tasks without being overwhelmed by excessive data or prompts. Attention and perception are aligned with the current demands, ensuring smooth task execution.

\myparagraph{Overload Scenarios} In high-pressure, overload scenarios where the pilot’s cognitive load is at its peak, the system reduces complexity by minimizing the amount of information delivered. Here, visual cues become the primary modality to prevent overloading the pilot with auditory or text-based distractions. The system focuses on essential tasks, providing only the most critical information to guide the pilot through urgent decision-making processes.
%This approach allows the pilot to focus on immediate priorities, reducing the risk of errors caused by cognitive overload, and ensuring their attention remains fixed on critical tasks.


% \subsubsection{Multi-modal Cues Adaptation}
\subsection{Adaptive Modality Selection}
The selection of the appropriate modality for delivering instructions ensures that the pilot receives information in a manner that is both effective and minimally disruptive. 
The system considers the pilot’s current cognitive state, including memory, attention, and perception levels, behavioral data, and task data. 
The objective is to ensure that transitions between modalities reduce cognitive disruption. 
The modalities available for instruction delivery include visual only, audio only, text only, visual and audio, visual and text, audio and text, and a combination of visual, audio, and text. By aligning the modality with the pilot’s cognitive state and the specific task at hand, the system aims to optimize the delivery of instructions, ensuring that the pilot can maintain focus and efficiency throughout the procedure.

Textual cues are presented via a pop up window in the pilots field of view. 
Visual cues are presented with a ghost hand pointing to the current action the pilot must perform. Audible cues are presented audibly to the pilot can be seen in Fig.\ref{fig:modality}
\begin{figure}
    \centering
    \includegraphics[width=1  \linewidth]{sections/Figures/modality.png}
    \caption{(a)is the tip window text cues;(b) is the visual cues}
    \label{fig:modality}
\end{figure}

\subsection{Dynamic Information Load}
% \subsubsection{Information Load Adaptation}
The system calibrates the information load based on the pilot’s cognitive state to avoid overwhelming them while ensuring that they remain engaged and focused. If the pilot is experiencing cognitive overload, the system limits the information load to essential command details only, minimizing the risk of further cognitive strain. In an optimal cognitive state, the system balances the information load by providing both command instructions and additional context, such as flight information or flight route details, which enhances the pilot’s understanding and situational awareness. When the pilot is underloaded, the system increases the information load by including comprehensive details, such as environmental updates, to ensure that the pilot remains engaged and maintains a high level of situational awareness. This dynamic adjustment of information load helps the pilot to remain focused and efficient without becoming overwhelmed or disengaged.

%lessons or formualtes 
\section{\systemname Implementation}

\subsection{Design Decisions}
\begin{figure}
    \centering
    \includegraphics[width=1  \linewidth]{sections/Figures/system.png}
    \caption{System design}
    \label{fig:system}
\end{figure}
To accommodate the complexity of the UH-60 Helicopters functionality \systemname is broken into two parts, the front-end VR system built in Unity, and the back-end system built in Python. Separating the two systems allows us to run the Unity build directly on the VR headset and perform complex calculations on a separate or even remote server as seen in fig.\ref{fig:system}.

\subsection{VR simulator for UH-60 Black hawk Cockpit}
Our test bed is built upon an existing high-fidelity UH-60 VR simulation. 
VR offers an easily configurable platform to adjust cockpit events and present information to the pilot. \cite{guthridge2023evaluating}. 
To match the real way a UH-60 pilot performs a pre-flight checklist \textcolor{red}{CITE}, the environment is modified to include an interact-able recreation of the paper checklist.

\subsection{Reasoning Model Selection}
To increase question reasoning and inference speed between pilot actions \systemname uses a quantized version of the Microsoft PHI-3 multi-modal large language model\cite{kaplan2020scaling}. the PHI-3 model is chosen for its good performance in question answering reasoning tasks\cite{kenton2019bert}. We choose a quantized version of the model to increase inference speed and for host ability on a local GPU server. \textcolor{red}{cite}

\subsection{Streaming Data}
To communicate between the front and back end data is streamed through the robot operating system (ROS) architecture \cite{koubaa2017robot}. ROS affords the system to be modularized into separate systems for separate functionalities. With this we run the PHI-3 LLM on a dedicated GPU cluster, the rest of the back end nodes on a dedicated computer, and the front end on the headset. Additionally, ROS provides a simple way to collect all data in the system through the use of the ROS BAG system. ROS BAGS record all data streams with normalized timestamps. This allows complete replay ability and extraction of data from a condition run. One issue with this separated design, is that if a error is made, there is a occasional disconnect between what the user thinks there step is and what the system thinks there step is.

\subsection{Error Dashboard}
To accommodate this disconnect between the front end and back end during errors. We provide a dynamic error dashboard to the user. This dashboard audibly alerts the pilot when a error is performed. The dashboard is placed outside the pilots field of view and each pilot was instructed to not use the dashboard unless they hear the audible error. If they hear the audible error, they were instructed to use the dashboard to get back on track with the system and then to transition back to paper checklist only. This introduces some additional cognitive load to the pilot however it is necessary for our system to track all actions that are performed.

\subsection{Functional Near-Infrared Spectroscopy}
The processing model for cognitive workload detection in pilots utilizes functional near-infrared spectroscopy (fNIRS) to continuously monitor and evaluate the pilot's cognitive state during flight operations. fNIRS is a non-invasive neuroimaging technology that measures brain activity by detecting changes in blood oxygenation levels within the cerebral cortex. This method is particularly effective in aviation environments due to its portability and ability to function in real-time, making it suitable for integration into pilot helmets or headsets.

FNIRS sensors are positioned to capture brain activity in the prefrontal cortex, associated with executive cognitive functions. The fNIRS device emits two wavelengths of near-infrared light into the scalp corresponding to oxygenated and deoxygenated hemoglobin.  The amount of light that is either absorbed or reflected back indicates a level of absorption that varies with the concentration of oxygenated and deoxygenated hemoglobin in the blood. This information is fed into a real-time workload prediction model to infer workload states and provide the PHI-3 reasoning model with information for appropriate adaptations.

% As the pilot engages in various tasks during different flight phases, the fNIRS system continuously records data, which is processed to assess three key aspects of the pilot's mental state: workload, attention, and perception. The workload is determined by analyzing the level of cognitive load the pilot is experiencing, inferred from the intensity of brain activity in the regions associated with task execution and problem-solving. High levels of sustained activity indicate cognitive overload, while low levels suggest underload, which may correspond to reduced engagement or vigilance.

% Attention is assessed by monitoring the pilot's focus and concentration on specific tasks or stimuli. This is achieved by detecting patterns of neural activity that correlate with sustained attention and task-oriented focus. If the fNIRS data indicates a diffuse or inconsistent pattern of activity, it may suggest that the pilot's attention is not fully engaged or is being diverted away from critical tasks.

% Perception, which refers to the pilot's ability to interpret and respond to the surrounding environment, is also evaluated through fNIRS. This is particularly important in dynamic flight conditions where the pilot must rapidly process and react to changing information. The fNIRS system detects the brain's response to sensory inputs and the integration of these inputs into a coherent situational awareness. High perception levels are associated with effective environmental monitoring and decision-making, while low levels may indicate difficulty in processing or interpreting sensory information.

% By continuously monitoring these parameters, the fNIRS system generates a real-time profile of the pilot's mental state, providing critical insights into their cognitive readiness and ability to handle the current flight demands. This information is then used to adapt the delivery of instructions and feedback, ensuring that communication is tailored to the pilot's current cognitive capacity, thereby enhancing performance and reducing the risk of errors.

\section{Pilot's Cognitive Load Modeling}

Predictions of the pilots' cognitive workloads, spanning working memory, attention, and perception, are derived from the fNIRS time series measurements of hemoglobin concentration. These measurements, captured at a frequency of 10 Hz, include raw light intensities, HbO (oxyhemoglobin), and HbR (deoxyhemoglobin) concentrations. These measurements serve as inputs for dedicated classifiers; at each time-step, three mental states are specified: perception, attention, and working memory. Each mental state is classified as either ``optimal'', ``overload'', or ``underload'' with an associated classification confidence (we elaborate upon the interpretation of these classes in the following paragraph). Each workload category has its own classifier, which runs concurrently during recording sessions. The classifiers are generalized mixed effects models trained on data gathered from a previous test bed study that showed cross-task and cross-participant transfer \cite{mckendrick_theories_2019}. The performer's classified mental state is first base-lined before recording and is not shown to the performer during collection.

Working memory capacity (which we hereafter refer to as \textit{memory}) is an individual's ability to retain and manipulate information during task execution. \textit{Attention} pertains to the individual's capacity to concentrate on specific tasks selectively. \textit{Perception} is the individual's ability to interpret stimuli, both visual and auditory. Each cognitive facet is categorizes into three states: optimal, overload, and underload. An optimal state denotes a balanced cognitive load conducive to task performance. An overloaded state suggests a cognitive burden exceeding an individual's capacity, potentially impairing the incorporation of new information~\cite{young_state_2015}. Conversely, an underloaded state indicates a cognitive engagement below the individual's capacity, which may result in diminished focus~\cite{young_state_2015}. It is critical to monitor multiple synchronous information streams alongside cognitive state data, as the presence of an overloaded or underloaded state does not invariably correlate with decreased task performance.

\section{PHI-3 Prompt Engineering}
The PHI-3 large language model is carefully prompt engineered to adapt guidance cues to the \systemname adaptive strategies. The reasoning model’s prompt structure is divided into three components: instructions, few-shot examples, and real-time context. The Instructions, given before execution, give PHI-3 context around the UH-60 cockpit from a tokenzied UH-60M operation manual. Additionally \systemname provides information regarding cognitive workload definitions and defines all adaptive strategies. The Few-shot examples provide the model with contextual examples of how to use the adaptive strategies on context to adapt guidance. Finally real-time context is given to the PHI-3 model during runtime. PHI-3 is given the pilots average cognitive workload across all 3 facets given the last 10 seconds, the pilots current tasks, and the pilots current gaze focus.

% Along with the cognitive workload state information we provide the Phi-3 LLM model with additional behavioral and task related information. Additionally we provide the LLM with a base prompt that includes a tokenzied version of a UH-60M operation manual,  Lastly, the LLM is instructed to provide a modality type (audio, visual, cue, or combination); a information load (information displayed to the user depending on type); and reasoning behind its choices.

% The reasoning model in the context of pilot training leverages a sophisticated approach to predict and adapt to the pilot’s cognitive and operational states, enhancing the accuracy and relevance of instructional outputs. By integrating real-time data from various sensors and employing a Chain-of-Thought (CoT) framework with advanced language models like Meta LLAMA, the system is capable of providing nuanced, contextually appropriate guidance that supports novice pilots in real-time.

% The reasoning model operates by first capturing and synthesizing multimodal data, including workload, attention focus, and procedural actions, into structured text. This data transformation is critical as it allows the system to integrate diverse inputs into a coherent format that can be processed effectively by the language model. The model then uses CoT prompting, a technique that involves breaking down the reasoning process into a series of intermediate steps. Each step builds upon the previous one, maintaining context and consistency throughout the decision-making process.

% In this approach, the reasoning model processes input data such as the current flight phase, the pilot’s mental state, and their interaction with the aircraft systems. The Chain-of-Thought framework is employed to guide the model through a series of logical reasoning steps, ensuring that the final instructional output is both accurate and aligned with the pilot’s immediate needs. The use of CoT enables the model to handle complex scenarios by considering each aspect of the pilot’s situation—cognitive load, attention distribution, and procedural context—before generating the output.

% \textbf{Task Context}
% %error made whether should use anaother section
% The task description plays a crucial role in understanding the pilot's interaction with the aircraft during pre-flight. This description is constructed by analyzing the pilot’s actions, procedures, and the current phase of flight. The system continuously monitors the flight phase and captures detailed information about the pilot's completed and ongoing procedures, as well as the specific actions that have been or need to be performed.

% The current procedure represents the task that the pilot is actively performing at the moment. In the ongoing example, the current procedure might be 'Confirm NAV DB / TAC DB,' where the pilot is required to verify the navigation and tactical databases on the CDU, ensuring that they are up to date and properly loaded. This procedure involves specific actions like pressing the appropriate line select keys (LSKs) to navigate through the CDU menus and visually confirming the data presented on the screen.

% The todo actions describe the steps the pilot needs to complete within the current procedure. These are detailed instructions that guide the pilot through the necessary interactions with the aircraft's systems. For instance, within the 'Load mission data' procedure, the todo actions might include 'Press LSK L2 LOAD MSN DATA,' 'Press LSK L5 LOAD ALL,' and 'Press LSK L5 CONFIRM.' These actions are sequential and must be performed accurately to complete the procedure successfully.

% Together, these elements—flight phase description, completed procedures, current procedure, todo actions, and last actions—provide a comprehensive overview of the pilot's current operational context. This detailed activity description allows the system to adapt its instructions and feedback, ensuring that the pilot receives relevant guidance. By closely monitoring the pilot’s progress and the specific actions they are taking, the system can help prevent errors, improve task execution, and support overall flight safety.

% The flight phase description identifies the current stage of the flight operation—preflight, climb/enroute, approach, or emergency. Each phase is characterized by distinct procedures and actions that the pilot must execute to ensure the aircraft's safe and efficient operation. For instance, during the preflight phase, the pilot might be involved in preparing the aircraft systems, loading mission data, and performing various checks to confirm that all systems are operational and correctly configured for the upcoming flight.

% Within this broader context, the completed procedures detail the specific tasks that the pilot has already accomplished. For example, if the pilot is currently engaged in the preflight phase, one of the completed procedures could be 'Load mission data.' This procedure involves a sequence of actions such as pressing the CDU INI key, selecting and confirming the loading of mission data through various soft keys on the control display unit (CDU).

% The last actions refer to the most recent steps the pilot has completed within the current procedure. This information is critical for maintaining continuity and ensuring that the pilot remains on track with the required tasks. For example, if the pilot has just completed 'Press LSK R4 DTS CTRL soft key' during the 'Load mission data' procedure, the system records this as the last action and updates the todo actions accordingly. The next step might involve pressing another LSK to continue the data loading process.


\subsubsection{Instruction}
The reasoning model is designed to provide adaptive instructions to novice flight trainees, ensuring that the guidance aligns with the pilot's current cognitive load, focus, and procedural context. The task of the reasoning model is to continuously assess and respond to the pilot's mental and operational state, adjusting the delivery of instructions to optimize learning and performance during flight training.

The instruction process is structured as follows:

\textit{"Given the current flight phase, cognitive load, attention focus, and the pilot's interaction with the UH-60 systems, determine the most effective modality and quantity of information to be delivered. This includes analyzing the pilot's completed and ongoing procedures, their last actions, and any errors that may have occurred. Based on this analysis, generate and deliver instructions that are clear, concise, and appropriate for the pilot's current state."}

\subsubsection{Few-shot Examples}
Four few-shot examples are provided to illustrate the functionality of our reasoning model in the context of pilot training. Each example consists of an input, a chain-of-thought reasoning process, and a corresponding output. We selected these examples to cover different cognitive states and procedural contexts within the preflight phase, including both error-free scenarios and situations where the pilot has made a mistake. This diversity ensures the model's adaptability across various conditions.

For each example, the input includes detailed descriptions of the pilot's ongoing procedures and the actions yet to be performed. Additionally, real-time cognitive workload state (working memory, attention, perception) levels—are captured, along with the pilot's gaze location.

\subsubsection{Reasoning}
The chain-of-thought reasoning process is constructed by defining the intermediate steps that the model should follow to generate the appropriate output. For instance, when the pilot experiences cognitive overload with optimal attention, the chain of thought involves assessing how this cognitive state might affect the pilot’s ability to execute the next steps accurately. The model is instructed to present this reasoning as part of its output.

% \subsubsection{Smoothing}
% In order to maintain a smooth transition between instructional modalities, the model employs a selection smoothing technique. This method ensures that the transition from one modality to another is consistent and logical, based on the modality used in the previous step.

% For example, if the pilot's previous instruction was delivered through the `audio` modality, the model will prioritize selecting `audio+visual` or `visual+text` for the next instruction, with a preference for `audio+visual`. This preference is based on the principle that maintaining some consistency in the modality (e.g., continuing to use audio) helps reduce cognitive load and disruption.

% The model calculates the likelihood of selecting a specific modality combination by considering the recent history of modality use, the pilot’s current cognitive state, and the task at hand. This calculated likelihood then guides the selection of the next modality, ensuring a smooth and coherent transition. If the modality combination in the current step is very similar to the one used in the previous step and the cognitive state remains stable, the model maintains the current modality setup.

% In this way, the selection smoothing technique reduces abrupt changes in instructional delivery, promoting a more fluid and consistent experience for the pilot. This approach is particularly beneficial during critical phases of flight, where maintaining continuity and minimizing cognitive shifts are essential.

% \subsubsection{Personalization}
% Our model incorporates a personalization mechanism that adapts based on the pilot's feedback and previous interactions. This method considers historical data on modality preferences and adjusts the current modality combination according to the pilot's cognitive state and task requirements. Specifically, the probability of selecting a modality combination is calculated using the following formula:

% \[
% \rho = \lambda_1 f + \lambda_2 g
% \]
% where \(\rho\) is the probability of selecting mode \(i\), \(f\) is the likelihood of pilots selecting this mode based on their feedback, and \(g\) represents the likelihood of smoothness in modality switching. The weights \(\lambda_1\) and \(\lambda_2\) are adjusted to balance between preference and smoothness.

% The personalization process involves evaluating the historical data of the pilot’s modality preferences. If a particular modality combination has been favored by the pilot in similar circumstances, it is prioritized. Additionally, the model ensures that transitions between modalities are smooth, thus minimizing cognitive disruption.

\subsubsection{Output}

The final output in each example includes the selected modality and the specific instructional load, tailored to the pilot's current cognitive workload state and task instructions. For the example, the instructions focus on reinforcing the next steps in a manner consistent with the pilot’s cognitive capacity.
\begin{itemize}
\item \textbf{Reasoning} The model provided reasoning as to why it chose the modality type and information load levels based on the provided cognitive workload levels, behavioral information, and task information.

\item \textbf{Modality Type} The modality type to use.

\item \textbf{Information load} The information to present to the pilot, for audio and text cues only.
\end{itemize}

% \subsubsection{Error handling}
% Error handling is an essential component of the instructional output generation process. If an error is detected in the pilot’s actions, the system immediately addresses it by informing the pilot of the mistake and providing corrective instructions. This feedback is designed to be clear and actionable, tailored to the pilot’s current mental state. For example, if the pilot presses the wrong button or follows the wrong steps, the system will notify them of the incorrect action and replay the correct procedure that needs to be performed. If no error is detected, the system continues with the next command instruction without additional correction. This approach ensures that the pilot receives timely and relevant feedback, which helps in correcting errors promptly and maintaining the flow of the task.
% \item \textbf{Information type}
% Once the modality is determined, the system proceeds to select the type of information that should be delivered to the pilot. This decision is directly influenced by the pilot’s current procedural step and cognitive state, ensuring that the information provided is both relevant and sufficient for task completion. The system categorizes information into several types: command instructions for specific aircraft operations, flight information such as airspeed, altitude, and fuel quantity, flight route information including navigation, tracking, and route modifications, and environmental information encompassing weather conditions and other relevant factors. The goal is to deliver information that is precisely tailored to the pilot’s needs at each step, thereby supporting effective task performance and maintaining situational awareness.

==> sections/test.tex <==
Our approach to adaptive guidance is neuroadaptive, meaning it adjusts based on cognitive workload theories to avoid overloading the pilot's attention, perception, or memory. We utilize 28 adaptive strategies, detailed in Appendix \cite{wickens2002multiple}, and base our rules on the following three key cognitive workload theories:
\begin{itemize}
    \item Underload Scenarios: Provide more information and use diverse modalities (visual, audio, text) to stimulate engagement and prevent errors due to a lack of focus. \cite{sweller1988cognitive}
    \item Overload Scenarios: Reduce the information load and rely primarily on visual cues to help reduce cognitive overload and keep pilots calm and focused. \cite{spence1997audiovisual}
    \item Optimal Scenarios: Use a balanced mix of visual and audio prompts, providing enough information to assist the pilot while avoiding unnecessary distractions. \cite{parasuraman2008mitigating}
\end{itemize}

To ensure effective adaptive guidance, we align our system with these cognitive workload theories. For instance:

\myparagraph{Underload Scenarios} In situations where pilots experience cognitive underload, the system increases engagement by providing more detailed information and introducing diverse modalities. Visual, audio, and text prompts are used to stimulate the pilot’s focus and ensure they remain attentive during less demanding phases of flight. As cognitive demand is low, introducing additional complexity helps prevent errors due to a lack of attention. 

\myparagraph{Optimal Scenarios} When the pilot’s cognitive load is in an optimal range, the system focuses on maintaining balance by providing a mixture of visual and audio prompts that are tailored to the task at hand. In these scenarios, the system aims to deliver just-in-time feedback, giving enough information to assist the pilot without causing distraction. 

\myparagraph{Overload Scenarios} In high-pressure, overload scenarios where the pilot’s cognitive load is at its peak, the system reduces complexity by minimizing the amount of information delivered. Here, visual cues become the primary modality to prevent overloading the pilot with auditory or text-based distractions. The system focuses on essential tasks, providing only the most critical information to guide the pilot through urgent decision-making processes.


\subsubsection{Multi-modal Cues Adaptation}
The selection of the appropriate modality for delivering instructions ensures that the pilot receives information in a manner that is both effective and minimally disruptive. 
The system considers the pilot’s current cognitive state, including memory, attention, and perception levels, behavioral data, and task data. 
The objective is to ensure that transitions between modalities reduce cognitive disruption. 
The modalities available for instruction delivery include visual only, audio only, text only, visual and audio, visual and text, audio and text, and a combination of visual, audio, and text. By aligning the modality with the pilot’s cognitive state and the specific task at hand, the system aims to optimize the delivery of instructions, ensuring that the pilot can maintain focus and efficiency throughout the procedure.

Textual cues are presented via a pop up window in the pilots field of view. 
Visual cues are presented with a ghost hand pointing to the current action the pilot must perform. Audible cues are presented audibly to the pilot can be seen in Fig.\ref{fig:modality}
\begin{figure}
    \centering
    \includegraphics[width=1  \linewidth]{sections/Figures/modality.png}
    \caption{(a)is the tip window text cues;(b) is the visual cues}
    \label{fig:modality}
\end{figure}

\subsubsection{Information Load Adaptation}
The system calibrates the information load based on the pilot’s cognitive state to avoid overwhelming them while ensuring that they remain engaged and focused. If the pilot is experiencing cognitive overload, the system limits the information load to essential command details only, minimizing the risk of further cognitive strain. In an optimal cognitive state, the system balances the information load by providing both command instructions and additional context, such as flight information or flight route details, which enhances the pilot’s understanding and situational awareness. When the pilot is underloaded, the system increases the information load by including comprehensive details, such as environmental updates, to ensure that the pilot remains engaged and maintains a high level of situational awareness. This dynamic adjustment of information load helps the pilot to remain focused and efficient without becoming overwhelmed or disengaged.

